How to Place Your Apps in the Fog -- State of the Art and Open Challenges

Fog computing aims at extending the Cloud towards the IoT so to achieve improved QoS and to empower latency-sensitive and bandwidth-hungry applications. The Fog calls for novel models and algorithms to distribute multi-service applications in such a way that data processing occurs wherever it is best-placed, based on both functional and non-functional requirements. This survey reviews the existing methodologies to solve the application placement problem in the Fog, while pursuing three main objectives. First, it offers a comprehensive overview on the currently employed algorithms, on the availability of open-source prototypes, and on the size of test use cases. Second, it classifies the literature based on the application and Fog infrastructure characteristics that are captured by available models, with a focus on the considered constraints and the optimised metrics. Finally, it identifies some open challenges in application placement in the Fog.

==> src/old_1_Introduction.tex <==
\section{Introduction}
\label{intro}
  
CISCO expects more than 50 billion of connected entities (people, machines and connected Things) by 2021, and estimates they will have generated around 850 Zettabytes of information by that time, of which only 10$\%$ will be useful to some purpose~\cite{cisco, cisco2}. As a consequence of this trend, enormous amounts of data -- the so-called \textit{Big Data}~\cite{bigdata} -- are collected by IoT sensors and stored in Cloud data centres~\cite{bigdataissues}. 
%
Once there, data are subsequently analysed to determine reactions to events or to extract analytics or statistics. Whilst data-processing speeds have increased rapidly, bandwidth to carry data to and from data centres has not increased equally fast~\cite{dustdar}. On one hand, supporting the transfer of data from/to billions of IoT devices is becoming hard to accomplish due to the volume and geo-distribution of those devices. On the other hand, the need to reduce latency for time-sensitive applications, to eliminate mandatory connectivity requirements, and to support computation or storage closer to where data is generated 24/7, is evident~\cite{buyyacomputer}. 

\medskip
In this context, a new utility computing paradigm took off, aiming at connecting the ground (IoT) to the sky (Cloud), and it has been named \textit{Fog computing}~\cite{bonomifog}. The Fog aims at better supporting time-sensitive and bandwidth hungry IoT applications by selectively pushing computation closer to where data is produced and by exploiting a geographically distributed multitude of heterogeneous devices (e.g.,  personal devices, gateways, micro-data centres, embedded servers) spanning the continuum from the IoT to the Cloud. \uib{Fig.~\ref{layerFogFig} shows three conceptual layers on current network infrastructure, where applications or services can be allocated in Cloud data centers or intermediate network devices.} %A substantial amount of computation, storage and networking is therefore expected to happen closer to where data is produced and to cyber-physical systems based on the IoT, contiguously to and interdependently with the Cloud. 
%
In its reference architecture\footnote{Very recently, the OFC reference architecture of Fog computing was adopted as the IEEE 1934-2018 standard \cite{ieee1934}.}, the OpenFog Consortium (OFC) \cite{openfogarch}, which is fostering academic and industrial research in the field since 2015, gives the following definition of Fog computing: 

\begin{center}
\it
Fog computing is a system-level horizontal architecture that distributes resources and services of computing, storage, control and networking anywhere along the continuum from Cloud to Things, thereby accelerating the velocity of decision making.  Fog-centric architecture serves a specific subset of business problems that cannot be successfully implemented using only traditional cloud-based architectures or solely intelligent edge devices.
\end{center}

%TODO DOUBLE-CHEK: Design?, reference in text?, caption?
\begin{figure}[bt]
\centering
\includegraphics[width=10cm]{img/modeloCEF.png}
\caption{\uib{Layer representation of Cloud and Fog architecture with application services allocated along the HW-devices}}
\label{layerFogFig}
\end{figure}


\noindent The NIST  has also recently proposed a conceptual architecture for Fog computing~\cite{nistconceptual}. Fog configures as a powerful enabling complement to the IoT+Edge and to the IoT+Cloud scenarios, featuring a new intermediate layer of cooperating devices that can autonomously run services and complete specific business missions, contiguously with the Cloud and with cyber-physical systems at the edge of the network~\cite{brogi2018bonsai}.

\medskip
Overall, Fog computing should ensure that computation over the collected data happens wherever it is \textit{best-placed}, based on various application (e.g., hardware, QoS) or stakeholders (e.g., cost, business policies) requirements. Since modern software systems are more and more often made from distributed, (numerous) interacting components (e.g., service-oriented and micro-service based architectures), it is challenging to determine where to deploy each of them so to fulfil all set requirements. 
%
\uib{The features of Fog architectures are quite different to cloud environments, mainly in the following points~\cite{moysiadis2018,DBLP:conf/fwc/MayerGSR17,doi:10.1002/cpe.5343}: (a) the Fog devices have limited resources, in contrast to data center nodes that have high computational and storage capacities; (b) the Fog devices are geographically distributed over wide areas throughout large-scale networks, in contrast to data center nodes that are located in the same geographic region; (c) the latency between the nodes of a data center is negligible, differing from fog domains where latency is a challenge; (d) nodes in data centers are usually connected via redundant links, in contrast to Fog networks, where regions of the network can be connected to the rest of the network with a single link, which, for example, could be a wireless one; and (e) fog devices are very heterogeneous devices, in contrast to data center devices, which usually have the same characteristics or very similar ones. These differences make it necessary to re-evaluate, or define new ones, traditional optimization policies. }
%
Lately, following this line, a significant amount of research has considered the problem of \textit{optimally} placing application functionalities (i.e., computation) based on different -- and sometimes orthogonal -- constraints. However, to the best of our knowledge, no comprehensive and systematic survey of these efforts exists in the literature.

This work aims precisely at offering an exhaustive overview of the solutions proposed for the application placement problem in the Fog, by providing the reader with \uib{two} complementary perspectives on this topic. Namely:
\begin{itemize}
\item[P1.] an \textit{algorithmic} perspective that reviews state-of-the-art contributions based on the methodologies that they employed to address Fog application placement, along with a study on the available prototypes and experiments,
\item[P2.] a \textit{modelling} perspective that analyses which (functional and non-functional) constraints and which optimisation metrics have been considered in the literature to determine best candidate application placements,
%\item[P3.] a \textit{future work} perspective that, based on both P1 and P2, identifies and discusses some of the open research challenges that should be studied on this topic.
\end{itemize}
\noident \uib{All the studies included in this paper are analysed and classified under these two perspectives. Additionally, and based on both P1 and P2, some of the open research challenges that should be studied on this topic are identified and discussed.}


The rest of this paper is organised as follows. After describing the methodology followed to realise this survey (Section \ref{settingthestage}), a comprehensive analysis of state-of-the-art related to Fog application placement under P1 (Section \ref{sect:algorithms}) and P2 (Section \ref{modelling}) is presented. Finally, some open problems and future research challenges that have been poorly addressed by the existing literature are pointed out (Section \ref{openchallenges}).



==> src/old_2_Stage.tex <==
This survey includes research articles that deal with Fog application placement with the objective of optimising non-functional requirements of the system. To set the stage, we start by formally defining the considered application placement problem.

\medskip
\textbf{Definition} -- Let $A$ be a multi-component \uib{(or multi-service)} application with a set of requirements $R$ and let $I$ be a distributed (Fog) infrastructure. Solutions to the \textit{Fog Application Placement Problem} (FAPP) are mappings from each component of $A$ to some computational node in $I$, meeting all requirements set by $R$ and optimising a set of objective metrics $O$ used to evaluate their quality. Solution mappings can be many-to-many, i.e. a component can be placed onto one or more nodes and a node can host more than one component.

%\bigskip

%  \noindent It is worth noting that FAPP can be solved or adjusted also at runtime (i.e., when $A$ is running), in case some requirements in $R$ cannot be met by the current solution mapping. In what follows, focusing on existing approaches to solve FAPP, we will exclude those works that only deal with dispatching or scheduling of (user or IoT) requests. Clearly, they represent a phase that is subsequent to the placement of the application components. Similarly, we will exclude research in the field of task offloading (i.e., outsourcing of the computation of a given function to get a result back) from one node to a better one (e.g., more powerful or reliable, closer), which is covered in detail by other recent surveys (e.g., \cite{aazam2018,xu2018}). 

%\noindent\textbf{Definition} -- Let $A$ be the set of multi-component applications that are deployed in the system with (hardware, software and QoS) requirements $R$. The applications are defined as a set of interacting modules or components $M$. Let $I$ be a distributed (Fog) infrastructure with interconnected nodes $N$ with computational capacities. Solutions to the \textit{Fog Application Placement Problem} (FAPP) are mappings from each component in $M$ to computational nodes in $N$, meeting all requirements set by $R$. Solution mappings can be many-to-many, i.e. a component can be placed onto one or more nodes and a node can host more than one component. Those solutions are addressed to optimise a set $O$ of metrics of the systems, while the considered constraints $C$ are satisfied.

\medskip
  \noindent It is worth noting that FAPP can be solved or adjusted also at runtime (i.e., when $A$ is running), in case that some requirements in $R$ cannot be met by the current solution mapping or whenever $O$ can be further optimised as Fog infrastructure conditions change over time. 

The concept of FAPP and the underlying technology are very recent, and the boundary with other technologies is not always clear. In this survey, we include all the articles that deal with the placement of applications that are generally available for the users and that \uib{can benefit from the adoption of the Fog computing paradigm.}
%have been traditionally requested to Cloud providers. 
%
Focussing on existing approaches to solve FAPP, we will exclude those works that only deal with dispatching or scheduling of (user or IoT) requests, as they represent a phase that is subsequent to the placement of the application components.
%
Similarly, we will exclude research in the field of task offloading (i.e., outsourcing of the computation of a given function to get a result back) from one node to a better (e.g., more powerful or reliable, closer) one, which is covered in detail by other recent surveys\cite{aazam2018,xu2018}. 

\uib{A problem similar to FAPP has been studied in the context of Software Defined Networking (SDN), and literature on the placement of Virtual Network Functions (VNFs) onto SDN substrates has been already thoroughly analysed in exhaustive recent surveys (e.g.~\cite{8066287,KARAKUS2017200,ASSEFA2019127,SALMAN2018221}). Such a problem is known as \textit{VNF embedding} and includes the joint placement of virtual function services and the routing of traffic flows between them. FAPP significantly differs from VNF embedding as it assumes to have the possibility of programming network flows from a (logically) centralised point of control in the infrastructure. As Fog application deployments will likely span various service providers, these might not always support SDN across their infrastructures, hence the previous assumption might be too stringent when considering Fog scenarios in general. Thus, also to avoid overlapping with existing surveys on SDN and VNF placements, in what follows, we will exclude results in those areas.
%commit our efforts to analyse the literature focussing on FAPP only.
}
%\uib{Works related to the use of software-defined networks to improve the QoS of Fog applications will be also excluded. This field is also analysed in respective surveys~\cite{8066287,KARAKUS2017200,ASSEFA2019127}} 
%
Finally, research in the field of mobile offloading, shifting the processing and execution from mobile terminals to the network or edges nodes, will be also excluded. 

\medskip
To the best of our knowledge, this is the first survey that covers the state of the art for FAPP. Our search criteria were formed by the following terms: {\sf (Fog computing $\wedge$ (service $\vee$ application) $\wedge$ (placement $\vee$ deployment))}. 
%
The search was carried out, with the help of Google Scholar, in the following libraries: IEEE Xplore Digital Library, Wiley Online Library, ACM Digital Library and Web of Science. To fully capture the advances in the field, both journal and conference articles were collected during the search phase. Additionally, the references in selected articles were also analysed to find more related work in the FAPP domain. 
%
At the end of this first step, the 110 articles we collected were carefully screened. After a more accurate and deeper selection process, where references in the field of offloading, dispatching, scheduling and VNF embedding were removed, we selected 38 articles to be analysed further. 

\medskip
%Table~\ref{tab:FAPPsummary} offers a complete overview of the set of the analysed papers with respect to all the factors that were included in our survey of the state of the art, showing the classification with respect to the algorithms and models employed in different works that approached FAPP. Focussing the definition of FAPP from an optimisation point of view, the common elements in any optimisation process are the following:

\uib{An overview of the set of the analysed papers with respect to all the factors that were included in our survey of the state of the art is offered in Figure~\ref{fig:algorithmbasedclassification} (algorithms),  Table~\ref{tab:FAPPsummaryalgorithm} (algorithms, solution's strengths and weaknesses, and availability of an open prototype), Table~\ref{tab:FAPPsummaryconstraints} (model constraints), and Table~\ref{tab:FAPPsummarymetrics} (optimisation metrics).} Focussing the definition of FAPP from an optimisation point of view, the common elements in any optimisation process are the following:


\begin{description}
\item{\bf Decision variables} They are the items whose values need to be determined during the optimisation process. In the case of the FAPP, they can be the binary decision variables (or, equivalently, the mapping functions) that indicate if a component of $A$ is allocated (or not) to a Cloud or Fog node of $I$. All the articles that we have included in our study rely on similar decision variables.

\item{\bf Objective function} The objective function measures the suitability of a solution (a specific value assigned to the decision variables) for the optimisation process. The optimisation can be addressed to maximise or minimise the value of the objective function. In a more general way, the objective function represents the concerns of the optimisation and defines the metrics that are optimised by fixing the values of the decision variables. In our case, the objective functions measure the metrics $O$ of candidate solutions to FAPP. 

\item{\bf Constraints over the decision variables} They define the requirements $R$ that must be satisfied by each specific case of the decision variables. Solutions (values of the decision variables) that do not satisfy the constraints are rejected as possible solutions to FAPP.

%They are presented in Section~\ref{sect:constraints}.

\item{\bf Domain variables or parameters} They commonly are the fixed values which are known previously to the optimisation process. But we also include here other variable, metrics or items related to the optimisation but that are not constraints neither optimisation objectives. 

%They are also presented in Section~\ref{sect:constraints} along with the constraints.

\item{\bf Algorithms} They are the algorithms proposed to find the values of the decision variables that achieve the best objective value while the constraints are satisfied. 
%
The problem of finding solution mappings between application components in $A$ and Fog/Cloud nodes in $I$, whilst minimising/maximising the values of the objectives functions $O$ and satisfying the constraints in $R$, is NP-hard. Moreover, when several opposite optimisation objectives are considered, it is necessary to determine a trade-off between the objectives because some of them may increase when the other decrease. Indeed, FAPP needs to be solved by evaluating -- at worst -- all the possible solutions, i.e., assuming the application is made of $m$ modules and the infrastructure is composed of $n$ nodes, $n^{m}$ different candidate solutions. 
%
Such complexity can be tamed by using heuristics which permit to find sub-optimal solutions. It is important to consider that Fog computing is a large-scale and dynamic domain, where real implementations have to deal with huge quantities of Fog nodes and applications.  
\end{description}

% \begin{table}
% 	\centering
% 	\caption{Articles according with the considered constraints and optimised metrics}\label{tab:FAPPsummary}

% 	%Scale the table to fit on the page: or this line or the next
%     \resizebox{0.98\columnwidth}{!}{
%   % \scalebox{0.6}{
%      \rowcolors{6}{white}{gray!20}
%      \begin{tabular}{@{}cc|cccc|cc|c|ccc|cc|c|c|ccc|c|c|@{}}\toprule
%   	%\begin{tabular}{@{}cccccccccccccccccccc@{}}\toprule
% %	\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}\toprule
    
% 	     &  & \multicolumn{10}{c|}{Considered Constraints}  & \multicolumn{8}{c|}{Optimised \& Comparison Metric(s)}& \\
%     	\cmidrule{3-12} \cmidrule{13-20} 
		
% %		&& \multicolumn{6}{c|}{Infrastructure} &  Energy &  \multicolumn{3}{|c}{Application}&& \multicolumn{8}{c}{}  \\
% %		\cmidrule{3-12} \cmidrule{14-21} 

% 	     & & \multicolumn{4}{c}{Network}&\multicolumn{2}{c}{Nodes}&\multicolumn{1}{c}{Energy}&
% 	    \multicolumn{3}{c|}{Application} &  \multicolumn{2}{c}{Network}&  Nodes&Energy&\multicolumn{3}{c}{Performance} &    Cost &\\
% 	\cmidrule{3-12} \cmidrule{13-20} 



% 		&Ref. & 
% 		%Constraints
% 		\multicolumn{1}{c}{\rotatebox[origin=c]{90}{Latency}} &
% 		\multicolumn{1}{c}{\rotatebox[origin=c]{90}{Bandwidth}} &
% 		\multicolumn{1}{c}{\rotatebox[origin=p]{90}{Link Reliability}} &
% 		\multicolumn{1}{c|}{\rotatebox[origin=c]{90}{Topology}} &
		 
% 		\multicolumn{1}{c}{\rotatebox[origin=c]{90}{Hardware}}&
% 		\multicolumn{1}{c|}{\rotatebox[origin=c]{90}{Software}}&
		  
% 		\multicolumn{1}{c|}{\rotatebox[origin=c]{90}{Energy}}&
		  		
% 		\multicolumn{1}{c}{\rotatebox[origin=c]{90}{Workload}}&
% 		\multicolumn{1}{c}{\rotatebox[origin=c]{90}{Dependencies}}&
		
% 		\multicolumn{1}{c|}{\rotatebox[origin=c]{90}{User preferences}}&

% 		%Optimization Objectives

		
% 		\multicolumn{1}{c}{\rotatebox[origin=c]{90}{Delay}}&
% 		\multicolumn{1}{c|}{\rotatebox[origin=c]{90}{Bandwidth}} &

% 	    \multicolumn{1}{c|}{\rotatebox[origin=c]{90}{Hardware}} &
	
% 	    \multicolumn{1}{c|}{\rotatebox[origin=c]{90}{Energy}} &
    
%     	\multicolumn{1}{c}{\rotatebox[origin=c]{90}{QoS-assurance}}&
% 	 	\multicolumn{1}{c}{\rotatebox[origin=c]{90}{Execution time}}&   
% 	  	\multicolumn{1}{c|}{\rotatebox[origin=c]{90}{Migrations}}&
% 		\multicolumn{1}{c|}{\rotatebox[origin=c]{90}{Cost}} &
%         \multirow{-3}{*}{\rotatebox[origin=c]{90}{Open prototype}}
%         %\multicolumn{1}{c|}{\rotatebox[origin=c]{90}{Prototype}}
%         \\\midrule
% %1 &2 & 3 & 4 & 5 & 6 & 7& 8 & 9 & 10 & 11 &  12 & 13 & 14 & 15 & 16 & 17 & 18 & 19 & 20& 21\\

% %% SEARCH ALGORITHMS
% \cellcolor{gray!10} &\cite{004} \cite{bookchapterbuyya}&\checkmark&\checkmark&&\checkmark&\checkmark&&&&&&\checkmark&\checkmark&&\checkmark&&\checkmark&&&\checkmark\\
% \cellcolor{gray!10}&\cite{021}&\checkmark&&&&\checkmark&&&&\checkmark&&&&&&\checkmark&&&&\checkmark\\
% %18
% \cellcolor{gray!10} &\cite{101}&\checkmark&&&\checkmark&\checkmark&&&\checkmark&\checkmark&&\checkmark&&&&&&&&\\
% %20
% \cellcolor{gray!10} &\cite{036}&\checkmark&\checkmark&&\checkmark&&&&\checkmark&\checkmark&&\checkmark&\checkmark&&&&&\checkmark&&\\
% %22
% \cellcolor{gray!10} &\cite{011}&\checkmark&\checkmark&&&\checkmark&\checkmark&&&&&&\checkmark&&&\checkmark&&&&\\
% %23
% \cellcolor{gray!10} &\cite{012}&\checkmark&\checkmark&&&\checkmark&\checkmark&&&&\checkmark&&\checkmark&&&\checkmark&&&&\checkmark\\
% \cellcolor{gray!10} &\cite{102} \cite{bookchapter}&\checkmark&\checkmark&&&\checkmark&\checkmark&&&&&&\checkmark&&&\checkmark&&&\checkmark&\\

% \cellcolor{gray!10} &\cite{109}&&&&&\checkmark&\checkmark&&&&&\checkmark&&&&&\checkmark&&&\\

% %29
% \cellcolor{gray!10} &\cite{032}&&\checkmark&\checkmark&&\checkmark&&&&\checkmark&&&&&&&&&\checkmark&\\
% %31
% \cellcolor{gray!10} &\cite{062}&\checkmark&\checkmark&&&\checkmark&&&&&&&&&&\checkmark&&&\checkmark&\\
% %32
% \multirow{-11}{*}{\rotatebox[origin=c]{90}{\cellcolor{gray!10} Search }} &\cite{027}&&\checkmark&&&\checkmark&&&&&&&\checkmark&\checkmark&\checkmark&&\checkmark&&&\\


% %% ILP ALG
% \cellcolor{white}& \cite{029}&&&&&&&&&&&\checkmark&&&&&&\checkmark&&\\
% %35
% \cellcolor{white}&\cite{001}&&\checkmark&&&\checkmark&&&\checkmark&\checkmark&&&&&&&&&\checkmark&\\
% %36
% \cellcolor{white}&\cite{034}&&&&\checkmark&\checkmark&&&\checkmark&\checkmark&&\checkmark&&\checkmark&&&&\checkmark&\checkmark&\\
% \cellcolor{white}&\cite{017}&&&&&\checkmark&&&&&&\checkmark&&&&&&&&\\

% %38
% \cellcolor{white}&\cite{095}&&&&&\checkmark&&&&\checkmark&&\checkmark&&&&&\checkmark&&&\\
% \cellcolor{white}&\cite{061}&\checkmark&&&&\checkmark&&&&&&\checkmark&&&&&&&&\\
% %42
% \cellcolor{white}&\cite{002}&\checkmark&\checkmark&\checkmark&\checkmark&\checkmark&&\checkmark&&&&&&&\checkmark&&&&&\\

% \cellcolor{white}&\cite{107}&&&&&\checkmark&&&\checkmark&&&&&&&\checkmark&&&&\checkmark\\
% \cellcolor{white}&\cite{024}&&&&\checkmark&\checkmark&&&&&\checkmark&&&\checkmark&&\checkmark&&&&\\
% \cellcolor{white}& \cite{025}&&&&\checkmark&\checkmark&&&&\checkmark&&&&\checkmark&&\checkmark&&&&\\\

% %47
% \cellcolor{white}&\cite{066}&&&&\checkmark&&&&&&&\checkmark&&&&&\checkmark&&\checkmark&\\
% \cellcolor{white}&\cite{019}&&&&\checkmark&&&&&&&&&&\checkmark&&&&&\\
% %49
% \cellcolor{white}&\cite{014}&\checkmark&&&&&&&&&&\checkmark&&&\checkmark&&\checkmark&&&\\


% %51
% \cellcolor{white}&\cite{030}&&\checkmark&&\checkmark&\checkmark&&&&&&&&&&\checkmark&&&&\\
% %54-%55
% \cellcolor{white}&\cite{105}\cite{106}&&&&&\checkmark&&&&&&&&&&\checkmark&&&&\checkmark\\
% \multirow{-16}{*}{\rotatebox[origin=c]{90}{\cellcolor{white} Mathematical Programming }} &\cite{038}&\checkmark&\checkmark&\checkmark&\checkmark&\checkmark&&&&&\checkmark&\checkmark&&&&&\checkmark&&&\checkmark\\


% %% OTHER ALGORITHM
% %60
% \cellcolor{gray!10} &\cite{033}&&&&&&&&&&&&&&&&\checkmark&&&\\
% %61
% \cellcolor{gray!10} &\cite{076}&&\checkmark&\checkmark&&\checkmark&&&&&&\checkmark&&&&&\checkmark&&&\\
% \cellcolor{gray!10} &\cite{053}&\checkmark&&&&&&&&&&&&&&&&&\checkmark&\\


% %64
% \cellcolor{gray!10} &\cite{088}&\checkmark&&&&&&&&&&&&\checkmark&&&&&&\\
% %66
% \cellcolor{gray!10} &\cite{008}&\checkmark&\checkmark&&\checkmark&\checkmark&&&&&&&&&\checkmark&\checkmark&\checkmark&&\checkmark&\\

% %67
% \cellcolor{gray!10} &\cite{064}&\checkmark&&&&\checkmark&&\checkmark&&&&&&\checkmark&\checkmark&\checkmark&&\checkmark&\checkmark&\\

% %69
% \cellcolor{gray!10} &\cite{006}&&&&&\checkmark&&&&\checkmark&&&\checkmark&&\checkmark&\checkmark&&&\checkmark&\\


% \multirow{-10}{*}{\rotatebox[origin=c]{90}{\cellcolor{gray!10} Other Algorithms}} & \cite{110} & &&&\checkmark&\checkmark&&&&&&\checkmark& &&&&&\checkmark&&\\
% \bottomrule

% 	\end{tabular}%

% }
% \end{table}


\medskip
\noindent Overall, we have organised the description and presentation of the articles from the point of view of the elements of the optimisation process: algorithms (Section~\ref{sect:algorithms}), constraints and parameters (Section~\ref{sect:constraints}), and objective functions, presented (Section~\ref{sect:objective}). \uib{Table~\ref{tab:FAPPsummaryalgorithm}, Table~\ref{tab:FAPPsummaryconstraints}, and Table~\ref{tab:FAPPsummarymetrics}} present a summary of the characteristics of the articles by following this organisation into algorithms, constraints and optimisation metrics.

The result of the analysis of the algorithms proposed in the articles has shown that seven different types of algorithm have been proposed to optimise FAPP. We have grouped and analysed the articles in Section~\ref{sect:objective} by those optimisation algorithms resulting in two main groups, with the highest number of articles proposing mathematic programming and heuristic/search solutions. The rest of algorithms have been only studied in a more reduced number of articles: bio-inspired algorithms, game theory, deep learning, dynamic programming, and complex networks.

\medskip
In the case of the constraints, we analysed the articles and classified the constraints into a two-level taxonomy. In a first level, we considered constraints related to the main elements in a Fog architecture: application, nodes (or Fog devices), network, and energy. With the analysis of the articles, we detected: network constraints related to the communication time (latency), bandwidth, link reliability, and the organisation and interrelation between the network components (topology), node constraints related to their hardware characteristics and the features of their operating systems or available frameworks (software), application constraints related to the type and number of requests that are generated in the systems (workload), the organisation and interrelation between application modules (dependencies), and the possibility of the users to establish conditions in the application placement or to choose between a set of placement alternatives (user preferences). The energy constraints are only related to the power consumption and a second classification was not considered for them.

\medskip
From the analysis of the optimisation objectives, we observed that the articles could be described by considering if they optimised or analysed metrics with respect to: the network, in particular, the delay due to the communication that is included in the execution time of the applications (network delay), and the usage of the network (network bandwidth), the nodes or devices, more specifically, the quantity of hardware resources that are consumed by the applications in the nodes (hardware), the energy, i.e., the power consumption that the execution of the applications generates in the Fog nodes, the performance of the system, and more concretely, the Quality of Service (QoS), commonly measured as the number of requests executed before a specific deadline (QoS-assurance), the execution time of the application requests (execution time), and the overhead that generates in the system the migration of application modules through the Fog nodes (migrations), and finally, the price to be paid for the use of the Fog resources (cost).



==> src/old_31_Algorithms.tex <==
\subsection{Algorithms}
 \label{sect:algorithms}

%  \begin{table}
%  \begin{minipage}{\columnwidth}
% 	\centering
% 	\caption{\uib{Brief summaries of the articles and a classification according with the considered algorithm}}\label{tab:FAPPsummaryalgorithm}

% 	%Scale the table to fit on the page: or this line or the next
%     \resizebox{0.5\columnwidth}{!}{
%   % \scalebox{0.6}{
%      \rowcolors{3}{gray!20}{white}
%      \begin{tabular}{@{}|c|c|p{0.5\columnwidth}|c|c|c|@{}}\toprule
%   	%\begin{tabular}{@{}cccccccccccccccccccc@{}}\toprule
% %	\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}\toprule
%          Ref. & Alg.\footnote{Alg.: S Search; MP Mathematical Programming; BI Bio-inspired; GT Game Theory; DL Deep Learnign; DP Dynamic Programming; CN Complex Networks} & Description & Strengths & Weaknesses & Open  \\
%           & &  &  &  & Proto. \\


%         \midrule
% %1 &2 & 3 & 4 & 5 & 6 & 7& 8 & 9 & 10 & 11 &  12 & 13 & 14 & 15 & 16 & 17 & 18 & 19 & 20& 21\\

% %% SEARCH ALGORITHMS
% \cite{004}\cite{bookchapterbuyya} & S &&&& \checkmark\\
% \cite{021} & S &They relocate the nodes according to the number of modules occupying a node and not exceeding a degree of use marked manually (60\%). With their method they waste nodes. They go through nodes with high demand and place modules in other nodes: the first fits solution. To solve the waste of nodes, they invent a period of observation that once overcome some nodes are turned off.&&& \checkmark\\
% %18
% \cite{101} & S &Guerrero and Lera proposed a decentralized algorithm for the placement of fog services. The algorithm used data local to the fog device to decide if it allocate the service of if the placement decission is shifted to other devices in the shortes path between the user/iot device and the cloud provider.&&& \\
% %20
% \cite{036} & S &Migration plan based on "Time-Graphs" weights= latency+bw&&& \\
% %22
% \cite{011} & S &The authors propose a modelling for Fog infrastructures and applications and a heuristic algorithm to determine eligible deployments of a given application to an available infrastructure. &&& \\
% %23
% \cite{012} & S &The authors extend their previous work [11] by including variations in the QoS of end-to-end links. Monte Carlo simulation is used to account for such variations when looking for eligible deployments.&&& \checkmark\\
% \cite{102}\cite{bookchapter} &S&It proposes a solution that finds all eligible placements of a multi-component application to a Fog infrastructure, matching app constraints to infrastructure capabilities. It exploits Monte Carlo simulations to account for variations in network QoS and to estimate how likely a deployment is to meet the app constraints. A cost model is proposed that merges costs coming from IoT, Cloud and Fog.&&& \\

% \cite{109} &S&With a model very close to the one of FogTorch, they proposed a backtracking solution to FAPP aimed at minimising the average response time of deployed IoT applications. Two new heuristics were devised. The first one sorts the nodes considered for deploying each component in ascending order with respect to the (average) latency between each node and the IoT devices required by the component. The second one dynamically considers a component that caused backtracking as the first one to be mapped in the next search step. A motivating IoT application \cite{doorbell} (i.e., 6 application components replicated up to $\simeq$ 800 times) was used to compare the exhaustive search, the first-fit (FF) algorithm, and the use of the two heuristics on very large infrastructures (i.e., 1 Cloud, up to $\simeq$ 20000 Fog nodes). Whilst the exhaustive search could not handle more than 150 nodes, the FF and the heuristic strategy scaled up to 20000 nodes, showing the latter a 40\% improvement on the the average response time of deployed applications with respect to FF. Prototype implementations were not released.&&& \\

% %29
% \cite{032} & S &They use a tree application structure (hierarchical set of processes), where ancestors have dependencies with descendants. They try to establish a cycle-free placement (physical graph) among the application nodes (application graph). On each physical node they consider CPU, storage and I/O. In the objective function they try to maximum the use of each physical node and link (avoiding overload and points of failures). Evaluation via simulation using 2 algorithms: greedily minimizes the maximum resource utilization and Vineyard algorithm.&&& \\
% % Search 31
% \cite{062} & S &They implement a deployment algorithm that it has two parts: "i) which request should be considered first and (ii) which device should be used for deployment first". Plus, they check these constraints: " Satisfied requests: The number of requests, which have been successfully deployed on the devices. Running time: The running time of the module deployment algorithm. Deployment time: The time taken by deploying the modules. Network traffic: The amount of network traffics produced by the modules." Testbed is a little onfuse but it is implemented using Kubernetes with several devices and with 3 types of modules (for one app).&&& \\
% %32
% \cite{027} & S &Modelling CPU, RAM and bandwidth requirements of app module, the proposed heuristic algorithm attempts to deploy each of them (i) to Fog nodes (sorted in descending order of free resources) and then (ii) to the Cloud. The experimental evaluation carried with iFogSim shows improvements in latency, energy consumption and network usage wrt Cloud-only deployments.The proposed solution has linearithmic complexity in the number of considered nodes (i.e., sorting them).&&& \\


% %% ILP ALG
%  \cite{029} &MP&The authors present a framework for service migration in the fog that is continuously evaluated accrdoing to the users and networks changes. The authors focussed the work in the implementation details of the service orchestrator and how it gathers the information from the system. But they only suggest some optimization solutions and they are not implemented.&&& \\
% %35
% \cite{001} &MP&The authors optimized VM placement and task distribution across fog devices with a mixed-integar non-linea program (MINLP), that was linearise to a MILP. Their objective was to minimize the communication and computation cost. Their solution also warrantied the QoS requeriments.&&& \\
% %36g.
% \cite{034} &MP&They refer to cloudlets. They define both a Service Placement Problem and a Cost-aware Service Placement Problem with the goal of optimising the trade-off between access latency, resource usage, and (data) migrations (costs). The solution consists of both (i) service placement and (ii) balanced request dispatching. The formulation accounts for constraints on the available resources as well as for workload variations depending on users' service accessing patterns. The proposed greedy heuristic (solving a relaxed problem and approximating a solution for the considered ones) outperforms other benchmark algorithms.&&& \\
% \cite{017} &MP&The authors improve the network latency (called communication cost) by defining a MINLP problem that manages the base station association, the task distribution and the VM deployment. The problem is linearized into an two-phase LP-problem.&&& \\

% %38
% \cite{095} &MP&The authors studied how to minimize the task completition time by considering a fog system where the task images are stored in storage servers and executed in computation servers. They focussed on simultaneously minimizing the I/O time and the computation time. They used a MILP approximation for the placement of the task images and their schedulling plan.&&& \\
% \cite{061} &MP&It models service allocation in Fog scenarios as an integer linear programming problem, aimed at optimising latency/delay needed for resource allocation. Resources are modelled uniformly as available slots at diffent nodes. Services are few requiring considerable amounts of resources (elephants, 10\%) and hundreds requiring few resources (mice, 90\%). They account both for sequential and parallel resource allocation.&&& \\
% %42
% \cite{002} &MP&&&& \\

% \cite{107} &MP&&&& \checkmark\\
% \cite{024} &MP&It proposes a hierarchical modelling of Fog landscapes, with a centralised management system to which control nodes of Fog colonies (IoT devices) connect. A ILP formulation of the problem of allocating computation to Fog cells is proposed to optimise QoS-assurance (i.e., time deadlines on app execution). IoT constraints are considered as type of resources (sensors/actuators) needed by an app to execute. Apps are associated to user-defined deadlines (which compares to the sum of makespan, comms delays and deployment time). The proposed approach is compared to first fit and Cloud-only deployment. Cloud cost is also taken into account, with linear growth.&&& \\
%  \cite{025} &MP&The authors propose a two level service management. They the defined a fog colony as a subset of fog devices with a fog control node which orchestrates the service placement. The control node select the fog device in the colony for the location of the service, or it migrates the service to a neighbording colony. The authors implemented a GA for the selection of the nodes. &&& \\

% %47
% \cite{066} &MP&&&& \\
% \cite{019} &MP&The authors modelled the problem of mapping services and devices as a quadratic programming problem, to afterwards simplified it to an integer programming problem and a weighted independent set (MWIS probelm). The services are modelled as a co-location graph, and heuristics are used to find the MWIS.&&& \\
% %49
% \cite{014} &MP&Tradeoff between power consumption and delay (network). The main problem is descomposed in three parts: power-delay vs fog.communication, power-delay vs cloud.communication, delay in WAN. Constraints: WL balanced, HW-nº working machines, Bw. Modelling using Markov (M/M/n) models. Simulation: Matlab. &&& \\


% %51
% \cite{030} &MP&The authors present a methodology to provide guidelines to developers at development and deployment phases to optimizae the performance and the utilization of the resources. The methodology is based in three phases: Benchmarking, Evaluation and Testing. The dea with the Fog Service Placement Probelm in a fog colony organization. &&& \checkmark\\
% %54-%55
% \cite{105}\cite{106} &MP&&&& \checkmark\\
% \cite{038} &MP&It models the placement problem as a linear problem, trying to optimise end-to-end application latency and availability. It considers scalar resource constraints at Fog nodes and user preferences (political, operator pinning). Placement of both computation modules and streams is considered. Response time and availability are optimised using a Simple Additive Weighting tecnique. Extensions to the model so to include bandwidth constraints and a network related objective function which includes network usage, traffic and elastic energy computation. The authors prototyped an Apache Storm extension (with CPLEX) and performed experiments, according to their model. Scalability of the approach is shown via experiments.&&& \\


% %% OTHER ALGORITHM
% %60
% \cite{033} &BI&This work is mainly a survey, but the authors devoted one section for an early optmization experience based on GA and parallel GA.&&& \\
% %61
% \cite{076} &BI&It models a hybrid cloud environment (similar to Fog) where nodes have constraints on CPU and memory, whilst links are bandwidth constrained. Node and links are associated to a failure probability. A minimum reliability and a maximum number of replicas is defined for each application (multi-service). A distributed genetic algorithm is applied, by using Biased Random-Key arrays to represent solutions (instead of binary arrays). The placement ratio is used to evaluate the proposed algorithm. GRECO shows near optimal results, shows faster execution time wrt ILP when there are constraints on availability and scales in the amount of duplicates but not of apps.&&& \\
% \cite{053} &GT&It models the allocation problem as Stackelberg games between data service subscribers and data service providers, the latter owning fog nodes. A first game is used to determine the number of computing resource blocks that users should purchase (based on latency requirements, block prices and utility). A second game is used to help providers set their prices so to maximise revenues. A matching game is used to map providers to fog nodes based on their preferences. And, finally, matching between fog nodes and subscribers is refined to be stable. &&& \\


% %64
% \cite{088} &GT&Similar to [17]. Service providers, Fog nodes and service subscribers. The mapping between the resources of Fog nodes and the service subscribers are modelled as a student allocation project. Subscribers consider revenues, data transmission costs, providers cost and latency to evaluate possible assignments. Providers consider revenue from subscribers minus cost of service delay.&&& \\
% %66
% \cite{008} &DL&Applications are hosted in containers, can be migrated (considering communication delay and computational power consumptions). They use a Markov Decision Process spaces. (delay, power consumption, and migration cost). SLA. Optimization alg.: Q-learning algorithm. Comparative: I) Testbed: VM and Containers migration. II) Real-world driver trace: San Francisco taxi traces: > mobile users!&&& \\

% %67
% \cite{064} &DP&The problem of service allocation to Fog nodes is modelled as a 0-1 multidimensional knapsack problem with the objective of (i) minimising allocation delay (ii) minimising average load of fog nodes (iii) minimising energy consumption. &&& \\

% %69
% \cite{006} &DP&A knapsack+symbiotic algorithm for task scheduling is proposed and run against iFogSim example. Comparison with FCFS and plain knapsack is provided.&&& \\


% \cite{110} &CN&&&& \\
% \bottomrule

% 	\end{tabular}%
% 	\newline

% }
% \end{minipage}
% \end{table}

%TODO DOUBLE-CHEK: Design?, reference in text?, caption?
\begin{figure}[bt]
\centering
\includegraphics[width=10cm]{img/section31.png}
\caption{\uib{Taxonomy for the classification of the studies in terms of their algorithms or methodologies for solving FAPP}}
\label{section31Fig}
\end{figure}





\begin{figure}[bt]
\centering

\begin{tikzpicture}[show/.style={circle,draw}]
\node[show, align=center]    (search)    at    (2,4)    
    [label=above:{Search-based Algorithms}]    
    {\cite{004} \cite{bookchapterbuyya} \cite{021}\\ \cite{101} \cite{036} \cite{011} \cite{012}\\ \cite{102} \cite{bookchapter} \cite{109}\\ \cite{032} \cite{062} \cite{027}};
\node[show, align=center]    (mp)   at     (0,1)    
     [label=below:{Mathematical Programming}]    
    {\cite{029} \cite{001} \cite{034} \cite{017}\\ \cite{095} \cite{061} \cite{002} \cite{107} \cite{024}\\ \cite{025} \cite{066} \cite{019} \cite{014}\\ \cite{030} \cite{105} \cite{106} \cite{038} };
\node[show,minimum size=4cm]    (other)   at     (4,1)    
     [label=below:{Other Algorithms}]    
    {};
\node[show]    (bio)   at     (4,2) 
     [label={[label distance=-3pt]above:{\tiny Bio-inspired}}]   
    {\cite{033} \cite{076}};
    
\node[show]    (game)   at     (3,1) 
     [label={[label distance=-3pt]above:{\tiny Game Theory}}]    
    {\cite{053} \cite{088}};
    
\node[show]    (deep)   at     (4,1) 
     [label={[label distance=-3pt]below:{\tiny Deep Learning}}]    
    {\cite{008}};
    
\node[show]    (dynamic)   at     (5,1) 
     [label={[label distance=-3pt]above:{\tiny Dynamic Prog.}}]    
    {\cite{064} \cite{006}};
    
\node[show, align=center]    (cn)   at     (4,0) 
     [label={[label distance=-3pt]below:{\tiny Complex Networks}}]    
    {\cite{110}};

\end{tikzpicture}


\caption{\uib{Classification of the studies in terms of their algorithms or methodologies for solving FAPP}}
\label{fig:algorithmbasedclassification}
\end{figure}

 \begin{table}
% \begin{minipage}{\columnwidth}
	\centering
	\caption{\uib{Brief summaries of the articles and a classification according with the considered algorithm}}\label{tab:FAPPsummaryalgorithm}

	%Scale the table to fit on the page: or this line or the next
    \resizebox{0.99\columnwidth}{!}{
   % \scalebox{0.6}{
     \rowcolors{3}{gray!20}{white}
     \begin{tabular}{@{}|c|c|p{0.7\columnwidth}|p{0.7\columnwidth}|c|@{}}\toprule
  	%\begin{tabular}{@{}cccccccccccccccccccc@{}}\toprule
%	\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}\toprule
         Ref. & Alg.\footnotemark[2] & Strengths & Weaknesses & Open  \\
          & &  &  &   Proto. \\


        \midrule
%1 &2 & 3 & 4 & 5 & 6 & 7& 8 & 9 & 10 & 11 &  12 & 13 & 14 & 15 & 16 & 17 & 18 & 19 & 20& 21\\

%% SEARCH ALGORITHMS
\cite{004}\cite{bookchapterbuyya} & S &Based on a validated simulator. Use of referenced applications. Detailed experiments.&Exclusive use of tree-based infrastructures. Experiments with a small scale.& \checkmark\\
\cite{021} & S &Distributed management of the services. Reduction of management overhead.& Lack of details on how to implement the architecture components in real-world.& \checkmark\\
%18
\cite{101} & S &Decentralized management. Service placement based on local data of each node.& Experiments with a small scale. Increase of the number of service migrations.&\\
%20
\cite{036} & S &User mobility is considered. Uncertainty of future placements is considered.&Use of simple prediction mechanisms.& \\

%26
%TODO Antonio & Stefano
\cite{011} & S &&& \\
%27
%TODO Antonio & Stefano
\cite{012} & S &&& \checkmark\\
%28,29
%TODO Antonio & Stefano
\cite{102}\cite{bookchapter} &S&&& \\

\cite{109} &S&Combination of two sophisticated heuristics. Short execution times.& Dynamic scenarios are not considered.& \\

%29
\cite{032} & S &Placement aware of the application graph. Extensive validation of the results. Decomposable solution for a distributed solution in the future. &High complexity of the algorithms. Only tree-based infrastructures considered.& \\
% Search 31
\cite{062} & S &Real-time and scalable algorithm. Solution implemented in a common platform (Kubernetes). &Low scale of the experiments due to the use of a real test-bed.& \\
%32
\cite{027} & S &Logarithmic complexity of the algorithm. General enough to be applied to a wide range of cases, allowing it to be used as benchmark for other studies. & Results only compared with the traditional cloud-based placement approach.& \\


%% ILP ALG
 \cite{029} &MP&Detailed definition of the Fog architecture and the service placement modules. Clear specification of the interactions between modules.&Details of the ILP algorithm are not provided. Experimental results are not evaluated.& \\

%35
\cite{001} &MP&
Cost minimization problem formulated as a mixed-integer non-linear programming with joint consideration of data consumer association, task distribution, and virtual machine placement.& %flabby
A good example of projection of a real modelling environment for the case study. Small umber of nodes in the topology. Characteristics of the example not provided.
& \\

%36
\cite{034} &MP&
A prediction system to adapt the service placement and load dispatching according with the user's mobility. Exhaustive study with two large data-sets.& A global view of the infrastructure is required.& \\


\cite{017} &MP&
& & \\


%37
\cite{095} &MP&Three objectives (I/O, computation and transmission time) are represented in a well-defined mixed-integer nonlinear programming problem.&No details about the computation cost of the algorithm. Analysis considering a static vision of the ecosystem.& \\
%38
\cite{061} &MP&Authors include the notion of a second fog layer in multi-tier hierarchical network to increase the allocation alternatives. &Small scenario for the experiments. Evaluation of only one criterion, the delay.& \\


%39
\cite{002} &MP&
The problem is analysed from the perspective of a minimum cost mixed-cast flow problem with a rigorous mathematical formulation. & Details of the simulation are not provided, so the reproducibility of the study is not warrantied. & \\

%40
\cite{107} &MP&Placement aware of the user expectations. Shorter execution times than the compared algorithms. Results validated with other three algorithms. &Need of exploring other application models. Need of testing the solution in real fog environment.& \checkmark\\


\cite{024} &MP& Distributed management via fog colonies/partitions. Periodically executions of the optimization model to reduce overhead.& Limited and small scale experimentation. Execution times not provided.& \\
 \cite{025} &MP&Distributed management via fog colonies/partitions. Precise problem statement. &Fitness function based on the satisfaction of the constraints instead of the optimization objectives.& \\

%47
\cite{066} &MP&Distributed management via fog colonies/partitions. Use of a real network topology.& Experiments with only one fog colony. Cost evaluation neglects the fog execution costs.& \\
\cite{019} &MP&Placement driven by the interaction of the services of an application and the latency of the infrastructure. Important reduction of the energy consumed in the network communication.&The experiments only analyse the network energy cost.& \\
%49
\cite{014} &MP&Distributed scheduling. Suitable for highly variable scenarios. & Mobility of users not considered.& \\


%51
\cite{030} &MP&Experiments performed with a real scenario of a Smart City. Extensive evaluation of the experiments. & Limited by the availability of a testbed. No clear application in scenarios with high levels of dynamism.& \checkmark\\
%54-%55


\cite{105}\cite{106} &MP& Experiments on Apache ecosystem: Storm and ZooKeeper &
The decisions taken by the proposed scheduling algorithm affect negatively the application availability when many operators are involved.
& 


\checkmark\\



\cite{038} &MP&Rigorous mathematical formulation of distributed stream processing applications. Integration in Apache Storm,& Run-time not supported in terms of a properly handling of input streams or execution environments with continuously changing properties.& \\


%% OTHER ALGORITHM
%60
\cite{033} &BI&It provides a perspective of future directions in IoT service orchestration challenges& The article is still in a initial stage: a superficial introduction of topics without an exhaustive inclusion of related works and in the same way, the authors present a case study.
 & \\
%61
\cite{076} &BI& Fault-tolerance and distributed pool model for the genetic formulation.& Scalability problems by a CPU extensive decoding.&   \\ 


\cite{053} &GT& Two formal pseudo-algorithms for parings resources among nodes, services and subscribers. & Static vision of the ecosystem. & \\



%64
\cite{088} &GT&Pricing analysis using Stackelberg game in a three-tier network model.& Dynamic strategies are not implemented.& \\
%66
\cite{008} &DL&A rigorous formulation of the ecosystem with a reinforcement learning algorithm. Experimentation model with real-world driver traces.& Excessive dependency of the thresholds.& \\

%67
\cite{064} &DP&Load and energy adaptive strategy according to the resource availability. &Limited and small scale experimentation.& \\

%69
\cite{006} &DP&The algorithm is partially based on ideas from the relation of organisms, which opens an exploratory research line in the field. &Benefits of the proposed algorithms evaluated over basic and simple heuristics.& \\


\cite{110} &CN&Migration-aware policy. Mobility of users is considered. Based on a already tested framework for cloud environments.& Small scale experiment scenario. Tree-based topology of the network.& \\
\bottomrule
\multicolumn{5}{}{\footnotemark[2]Algorithm: S Search; MP Mathematical Programming; BI Bio-inspired; GT Game Theory; DL Deep Learning; DP Dynamic Programming; CN Complex Networks}\\

	\end{tabular}%
	\newline

}
%\end{minipage}
\end{table}



%UPI

In this section, all reviewed approaches are analysed according to the algorithms or methodologies that they use for solving FAPP. We identified three main classes of algorithms which have been exploited in the literature \uib{(Figure~\ref{section31Fig}, Figure~\ref{fig:algorithmbasedclassification} and Table~\ref{tab:FAPPsummaryalgorithm})}. Namely:

\begin{itemize}
\item \textit{search-based} algorithms, such as (heuristic) backtracking search, or first- and best-fit application placement, %or genetic algorithms,
\item \textit{mathematical programming} algorithms, such as integer or mixed integer linear programming,
\item \textit{other} algorithms like game theoretical or deep learning.
\end{itemize}

\noindent The rest of this section is organised according to this classification with the goal of providing the reader with a complete overview of the state of the art related to frameworks used for solving FAPP (Sections \ref{search_algs} to \ref{other_algs}). For each reviewed approach, we indicate the availability of open source research prototypes and the size of the experiment used for assessing or testing it.



\subsubsection{Search-based Algorithms}\label{search_algs}

Being FAPP an NP-hard problem, the first solutions which have been exploited to solve it are traditional search algorithms along with greedy or heuristic behaviour \cite{aima}. 

\medskip

%IFogSim
Among the first proposals investigating this direction, Gupta et al.\cite{004} and Mahmud et al.\cite{bookchapterbuyya} proposed a Fog-to-Cloud search algorithm as a first way to determine an eligible (composite) application placement of a given (Directed-Acyclic) IoT application to a (tree-structured) Fog infrastructure. The search algorithm proceeds Edge-ward, i.e. it attempts the placement of components \textit{Fog-to-Cloud} by considering hardware capacity only, and allows merging homologous components from different application deployments. An open-source tool -- iFogSim -- implementing such strategy has been released and used to compare it with \textit{Cloud-only} application placement over two quite large use cases from VR gaming (3 application components scaled up to 66, 1 Cloud, up to 80 Fog nodes) and video-surveillance (4 application components, scaled up to 19, 1 Cloud, up to 17 Fog nodes). Building on top of iFogSim, Mahmud et al.\cite{021} refined the Edge-ward algorithm to guarantee the application service delivery deadlines and to optimise Fog resource exploitation. 

\medskip
%UIB
Recently, exploiting iFogSim, Guerrero et al.\cite{101} proposed a distributed search strategy to find the best service placement in the Fog, which minimises the distance between the clients and the most requested services. Each Fog node takes local decision to optimise the application placement, based on request rates and free available resources. The \textit{SocksShop} \cite{weaveworks2016shocksshop} application (9 components) is used to evaluate the proposed decentralised solution against the Edge-ward policy of iFogSim --varying the replication factor in the range $1-5$  and the number of Fog nodes in the range $1-25$. The results showed a substantial improvement in network usage and service latency for the most frequently requested services. Also, Ottenwalder et al.\cite{036} proposed a distributed solution -- MigCEP -- both to FAPP and to runtime migration. Such proposal reduces the network usage in Fog environments and ensures end-to-end latency constraints by searching for the best migration, based on probabilistic mobility of application users. The OMNeT++ \cite{omnet} simulator was used to show how MigCEP improves live migration against a static and a greedy strategy over a dynamic large-scale infrastructure (i.e., 1000 emulated connected cars). No codebase was released for either the works of Guerrero et al.\cite{101} or Ottenwalder et al.\cite{036}.

\medskip
%UPI
In this context, Brogi and Forti\cite{011} proposed both an exhaustive and a greedy backtracking algorithm to solve FAPP based on the (hardware, software, IoT and QoS) requirements of multi-component applications, as well as to estimate QoS-assurance, resource consumption in the Fog layer \cite{012} and monthly deployment cost~\cite{102} of eligible placements. The devised approach works on arbitrary application and infrastructure graph topologies. The greedy heuristic attempts the placement of components sorted in ascending order on the number compatible nodes (i.e., \textit{fail-first}), considering candidate nodes one by one sorted in decreasing order on the available resources (i.e., \textit{fail-last}). 
%
QoS-assurance is estimated by means of Monte Carlo simulations so to consider variations in the QoS of end-to-end communication links and to predict how likely each application placement is to comply with the desired network QoS \cite{012}. An open-source prototype -- FogTorch$\Pi$ -- implementing the whole methodology has been released and used on different simple use cases (i.e., 3 application components, 2 Clouds, 3 Fog nodes) from smart agriculture and smart building scenarios. Despite exploiting worst-case exponential-time algorithms, the prototype was shown to scale \cite{bookchapter} also on the larger VR game example proposed by Gupta et al.\cite{004}. FogTorch$\Pi$ was also modularly extended by other researchers to simulate mobile task offloading in Edge computing \cite{demaio}.

\medskip
Significantly inspired by Brogi and Forti\cite{011}, Xia et al.\cite{109} proposed a backtracking solution to FAPP to minimise the average response time of deployed IoT applications. Two new heuristics were devised. The first one sorts the nodes considered for deploying each component in ascending order with respect to the (average) latency between each node and the IoT devices required by the component. The second one considers a component that caused backtracking as the first one to be mapped in the next search step. A motivating IoT application \cite{doorbell} (i.e., 6 application components replicated up to $\simeq$ 800 times) was used to assess the algorithms on very large random infrastructures (i.e., 1 Cloud, up to $\simeq$ 20000 Fog nodes). The exhaustive search handled at most 150 nodes, whilst the first-fit and the heuristic strategy scaled up to 20000 nodes, the latter showing a 40\% improvement on the response time with respect to first-fit. Prototype implementations were not released.



\medskip
%similar to UPI
Limiting their work to linear application graphs and tree-like infrastructure topologies, Wang et al.\cite{032} described an algorithm for optimal online placement of application components, with respect to load balancing. The algorithm searches for cycle-free solutions to FAPP, and shows quadratic complexity in the number of considered computational nodes. %Indeed, the solution relies on auxiliary data structures containing the costs of all pairwise mappings of a component to a given node, which are then searched for the best placement. 
An approximate extension handling tree-like application is also proposed, which considers placing each (linear) branch of the application separately and shows increased time complexity. The approach is simulated on 100 applications to be placed featuring 3 to 10 components each and infrastructures with 2 to 50 nodes. Finally, the achieved performance is compared against the Vineyard algorithm \cite{vineyard} and a greedy search minimising resource usage.

\medskip
Hong et al.\cite{062} proposed a (linearithmic) heuristic algorithm that attempts deployments prioritising placement of smaller applications to devices with less free resources. A face detection application made from 3 components is used to evaluate the algorithm on a small real testbed (1 server acting as Cloud, 5 Fog nodes). Along the same line, Taneja and Davy\cite{027} proposed a similar search algorithm that assigns application components to the node with the lowest capacity that can satisfy application requirements, also featuring linearithmic time complexity in the number of considered nodes. Binary search on the candidate nodes is exploited as a heuristic to find the best placement for each component, by attempting deployment to Fog nodes first (i.e., Fog-to-Cloud). The medium-scale experiments (i.e., 6 application components, 1 Cloud, up to 13 Fog nodes) were carried in iFogSim, but the code to run them has not been made publicly available.


\medskip

\subsubsection{Mathematical Programming}\label{lp_algs}

Mathematical programming \cite{mathematicalprogramming} is often exploited to solve optimisation problems by systematically exploring the domain of an objective function with the goal of maximising (or minimising) its value, i.e., identifying a best candidate solution. Many of the reviewed approaches tackled FAPP with such a mathematical framework, relying on Integer Linear Programming (ILP), Mixed-Integer Linear Programming (MILP) or Mixed-Integer Non-Linear Programming (MINLP).

\medskip
Velasquez et at.\cite{029} proposed a framework and an architecture for application placement in Fog computing. An ILP implementation is suggested but it is not realised nor evaluated by the authors. On the other hand, Arkian et al.\cite{001}, in addition to proposing a Fog architectural framework, formulated FAPP as a MINLP problem, where application components (i.e., VMs) are to be deployed to Fog nodes so to satisfy end-to-end delay constraints. The problem is then solved (along with the problem of task dispatching) by linearisation into a MILP and the solution is evaluated on data traces from IoT service demands (from 10-100 thousand devices) in the province of Teheran, Iran. The results of the experiment showed that the Fog promises to improve latency, energy consumption and costs for routing and storage. 
%
Similarly, Yang et al.\cite{034} tackled both FAPP and its cost-aware extension with the problem of balancing request dispatching. The proposed methodology attempts optimising the trade-off between access latency, resource usage, and (data) migrations (costs). It accounts for constraints on the available resources as well as for workload variations depending on users' service accessing patterns. A novel greedy heuristic (solving a relaxed LP problem and approximating a solution for the full-fledged ones) is shown to outperform other benchmark algorithms (i.e., classic ILP and GA) both in terms of obtained results and algorithm execution time over an example with 20 Fog nodes and 30 services to be placed.

\medskip
Alike to these proposals, Gu, Zeng et al.\cite{017, 095} solved FAPP along with task scheduling, converting a MINLP into a MILP, solved with the commercial tool Gurobi \cite{gurobi}. A simulation and comparison is provided against server-greedy (i.e., Cloud-ward) and client-greedy (i.e., Edge-ward) placement strategies, showing good improvements on response time when using the proposed approach in a medium (i.e., 15 to 25 application images, 11 Fog/Cloud servers\cite{095}) and large (i.e., 45 to 80 Fog nodes\cite{017}) sized use case.
%
Still relying on Gurobi (together with PuLP \cite{mitchell2011pulp}), Souza et al.\cite{061} solved FAPP as an ILP problem, aimed at optimising latency/delay needed for resource allocation. Resources are modelled uniformly as available slots at different nodes. Out of the services to be deployed, few of them were considered to require large amounts of resources (i.e., \textit{elephants}, 10\%) and many more required instead few resources (i.e., \textit{mice}, 90\%). In the experimental settings (90 applications, 1 Cloud, 6 Fog nodes) both sequential and parallel resource allocation were considered and the benefit of Fog computing was shown in terms of reduced delays in service access. 

\medskip
Alternatively, Barcelo et al.\cite{002} combined FAPP with the routing of requests across an IoT-Cloud (i.e., Fog) infrastructure. They modelled FAPP as a minimum (energy) cost mixed-cast flow problem, considering unicast downstream and multicast upstream, typical of IoT. Solution to FAPP is then provided by means of known poly-time algorithms, which are simulated via the LP solver Xpress-MP \cite{xpressmp} on mock data traces from three use cases (i.e., smart city, smart building, smart mobility). The experiments simulated tens of devices and showed some performance improvements  (as per latency, energy, reliability) with respect to traditional IoT deployments that do not rely on Fog nodes. Mahmud et al.\cite{107} proposed instead a QoE extension of iFogSim -- based on an ILP modelling of users expectation -- which exploited fuzzy logic and achieved improvements in network conditions and service quality.

\medskip
Skarlat et al. designed a hierarchical modelling of Fog infrastructures, consisting of a centralised management system to control Fog nodes organised per \textit{colonies}\cite{024, 025, 066}. Particularly, Skarlat et al.\cite{024} adopted an ILP formulation of the problem of allocating computation to Fog nodes in order to optimise (user-defined) time deadlines on application execution, considering IoT devices needed to properly run the application. A simple linear model for the Cloud costs is also taken into account. The proposed approach is compared via simulation to first-fit and Cloud-only deployment strategies, showing good margins for improvement, on a medium-sized use case (i.e., up to 80 services, 1 Cloud, 11 Fog nodes). 

\medskip
Some of the methodologies proposed in the literature combine ILP with other optimisation techniques. Huang et al.\cite{019}, for instance, modelled the problem of mapping IoT services to Edge/Fog devices as a quadratic programming problem, afterwards simplified into an ILP and into a Maximum Weighted Independent Set (MWIS) problem. The services are described as a co-location graph, and heuristics are used to find a solution that minimises energy consumption. A (promising) evaluation is performed over large-scale simulation settings (i.e., 50 services, 100 to 1000 Fog nodes). 

 \medskip
Similarly, Deng et al.\cite{014} followed a hybrid approach to model FAPP and to determine the best trade-off between power consumption and network delays (exploiting $M/M/n$ Markov models to describe network capabilities). After decomposing FAPP into three sub-problems (power-delay vs fog communication, power-delay vs cloud communication and minimising WAN delay) balanced workload solutions are looked for exploiting different optimisation methods (i.e., convex optimisation, generalised Benders' decomposition and Hungarian method). A quite large simulation setup in MATLAB \cite{matlab} was used to evaluate the proposed approach (i.e, from 30000 to 60000 nodes).

\medskip
Unfortunately, none of the approaches previously discussed in this section released the code to run the experiments. Conversely, based on the hierarchical model of Skarlat et al.\cite{025}, Venticinque and\cite{030} proposed a software platform to support optimal application placement in the Fog, within the framework of the CoSSMic European Project \cite{cossmic}. Envisioning resource, bandwidth and response time constraints, their approach permits to choose among a Cloud-only, a Fog-only or a Cloud-to-Fog deployment policy, which were evaluated in a small testbed (i.e., 1 Cloud, 1 Fog node) where a composite application (8 components) from Smart Energy scenarios \cite{cosmic_app} was deployed and run over emulated IoT data traces.

\medskip
Finally, Cardellini et al.\cite{105, 106, 038} discussed and released S-ODP, an open-source extension of Apache Storm that solves FAPP by means of the CPLEX \cite{ibmcplex} optimiser with the goal of minimising end-to-end application latency and availability of stream-based applications. Extensive experiments (i.e., up to 50 application components and up to 100 Fog nodes) showed scalability of the ILP approach (with respect to a traffic-aware extension of Storm \cite{xu_cardellini}), which can be easily extended to include bandwidth constraints and a network-related objective function considering network usage, traffic and elastic energy computation.


%\subsubsection{Genetic Algorithms}\label{ga_algs}


\subsubsection{Other Algorithms}\label{other_algs}
\begin{description}

\item[Bio-inspired Algorithms] Genetic algorithms (GAs) implement meta-heuristics to solve optimisation and search problems based on bio-inspired operators such as mutation, crossover and selection \cite{geneticalgorithms}. Naturally, some of the reviewed works exploited such bio-inspired search algorithms to explore the solution space of FAPP, and to solve it. Wen et al.\cite{033} surveyed Fog orchestration-related issues and offered a first description of the applicability of GAs and parallel GAs to FAPP.

Retaking the ILP model of Skarlat et al.\cite{024} based on Fog colonies and hierarchical control nodes, Skarlat et al.\cite{025} also proposed a GA solution implemented in iFogSim and compared to a greedy (first-fit) heuristic and to an exact optimisation obtained with CPLEX, over a small example (i.e., 5 application components, 10 Fog nodes). Whilst the first-fit strategy does not manage to guarantee user-defined application deadlines, both the exact solution and the GA do. Overall, the GA solutions are on average 40\% more costly than the optimal ones, despite guaranteeing lower deployment delays. 

Mennes et al.\cite{076} required the user to provide a minimum reliability measure and a maximum number of replicas for each (multi-component) application to be deployed. It employed a distributed GA, by using Biased Random-Key arrays to represent solutions (instead of binary arrays). The placement ratio (placed/required) is used to evaluate the proposed algorithm., which showed near-optimal results against a small example (i.e., 10 applications, 5 Fog nodes) and faster execution time with respect to ILP solvers.
%
Regrettably, open-source implementations are not provided for any of the works exploiting GA.

\medskip
\item[Game Theory] 

Game theoretical models \cite{gametheory} -- which describe well multi-agent systems where each agent aims at maximising its profit whilst minimising its loss -- were fruitfully applied to solve FAPP in \cite{053} and \cite{088}.

Zhang et al.\cite{053} modelled FAPP as Stackelberg games between data service subscribers and data service providers, the latter owning fog nodes. A first game is used to determine the number of computing resource blocks that users should purchase (based on latency requirements, block prices and utility). A second game is used to help providers set their prices so to maximise revenues. A matching game is used to map providers to Fog nodes based on their preferences. And, finally, matching between fog nodes and subscribers is refined in order to be stable. The proposal was tested in a simulated MATLAB environment considering 120 service subscribers, 4 data providers, and 20 Fog nodes.

Similarly, Zhang et al.\cite{088} describe a game among service providers, Fog nodes and service subscribers. The mapping between the Fog resources and service subscribers is determined to solve a student-to-project allocation problem. During the game, subscribers consider revenues, data transmission costs, providers' costs and latency to evaluate possible assignments. On the other hand, providers consider revenue from subscribers minus the cost of service delay.

\medskip
\item[Deep Learning] Reinforcement learning trains software agents (with reward mechanisms) so that they learn policies determining how to react properly under different conditions  \cite{deeplearning}.  To the best of our knowledge, only Tang et al.\cite{008} exploited recent reinforcement learning techniques to solve FAPP. After defining a multi-dimensional Markov Decision Process to minimise communication delay, power consumption and migration costs, a (deep) Q-learning algorithm is proposed to support migration of application components hosted in containers or VMs. The proposal took into account user mobility and was evaluated over a medium-sized infrastructure (i.e., $\simeq$ 70 nodes) using real data about users mobility taken from San Francisco taxi traces.

\medskip
\item[Dynamic Programming]

Differently from the others, Souza et al.\cite{064} modelled FAPP as a 0-1 multidimensional knapsack problem \cite{cormen}  with the objective of minimising a given objective function. Limited simulation results on a medium-sized example (40 application components, 6 Fog nodes, 3 Clouds) are provided by the authors. However, no details are given on how the solution is computed, and the code to run the experiments is not available.

Also Rahbari et al.\cite{006} modelled FAPP as a knapsack problem, by considering the allocation of application modules to running VMs in a Fog infrastructure. iFogSim was used to simulate the proposed symbiotic organisms search algorithm, showing some improvements in energy consumption and network usage with respect to a First Come First Served allocation policy and traditional knapsack solvers.

\medskip
\item[Complex networks] 
To the best of our knowledge, only Filiposka et al.\cite{110} relied on network science theory to model and study FAPP, employing on a community detection method to partition the available Fog nodes into a hierarchical dendogram\cite{barabasi}. The dendrogram was then used to analyse different community partitions so to find the most suitable set of nodes to support the VMs that encapsulate the applications. The proposal was validated with CloudSim \cite{cloudsim} over a quite large use case (i.e., 80 Fog nodes, and from 150 to 250 application components). The proposed community-based extension to CloudSim is, however, not available.


\end{description}
















